Sustainable Federated Learning

Potential environmental impact of machine learning by large-scale wireless networks is a major challenge for the sustainability of future smart ecosystems. In this paper, we introduce sustainable machine learning in federated learning settings, using rechargeable devices that can collect energy from the ambient environment. We propose a practical federated learning framework that leverages intermittent energy arrivals for training, with provable convergence guarantees. Our framework can be applied to a wide range of machine learning settings in networked environments, including distributed and federated learning in wireless and edge networks. Our experiments demonstrate that the proposed framework can provide significant performance improvement over the benchmark energy-agnostic federated learning settings.

==> 05_Experiments.tex <==





%%%%%%%%%%%%%%%%%%%%%%%%%%%



We now demonstrate the convergence properties of Algorithm~\ref{Alg} compared to  federated learning benchmarks that are agnostic to the energy availability of the clients. 

{\bf Network architecture.} We consider an image classification task with $10$ classes on the CIFAR-10 dataset \cite{krizhevsky2009learning}. 
% , distributed over 40 clients uniformly at random (i.i.d.).  
Training is done using a convolutional neural network with the same architecture from  \cite{mcmahan2017communication} (about $10^6$ parameters). 

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/plot-FL-v3.png}
\vspace{-0.6cm}\caption{Test accuracy of Algorithm~\ref{Alg} compared to federated learning benchmarks  for $N=40$ clients on the CIFAR-10 dataset. }
\label{fig:test-accuracy}
\vspace{-0.6cm}
\end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/plot-final-v2.png}
% \vspace{-0.6cm}\caption{Test accuracy of Algorithm~\ref{Alg} compared to federated learning benchmarks  for $N=40$ clients on the CIFAR-10 dataset. }
% \label{fig:test-accuracy}
% \vspace{-0.6cm}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.95\linewidth]{figures/plot-final.png}
% \vspace{-0.3cm}\caption{Test accuracy of Algorithm~\ref{Alg} compared to the federated learning benchmarks for $N=40$ clients on the CIFAR-10 dataset. }
% \label{fig:test-accuracy}
% \vspace{-0.2cm}
% \end{figure}


{\bf Experiment Setup.} We consider a network of $N=40$ clients. The dataset is distributed in an i.i.d. fashion across the network, by shuffling the dataset and distributing it evenly across the clients. Clients use the ADAM optimizer \cite{kingma2014adam} during training, and the number of local training iterations is set to $T=5$.   

% In our experiments, we consider a conventional image classification task with $10$ classes on the CIFAR-10 dataset \cite{krizhevsky2009learning}, distributed over 40 clients uniformly at random. Training is performed via distributed SGD using the convolutional neural network architecture from  \cite{mcmahan2017communication} (about $10^6$ model parameters).  

{\bf Energy Profile.} In order to show the impact of non-homogeneous energy arrivals, clients are partitioned into $4$ groups $\mathcal{U}_0, \ldots, \mathcal{U}_3$ of equal size, such that  $\mathcal{U}_ k =\{i: i\mod 4 = k\}$. Then, the energy arrivals of clients in group $\mathcal{U}_k$ are assigned as $E_i = \tau_k$ for all $i\in\mathcal{U}$, where $(\tau_0, \tau_1, \tau_2, \tau_3) = (1, 5, 10, 20)$. 
In other words, clients in group $\mathcal{U}_0$ receive energy at every global round, whereas clients in groups  $\mathcal{U}_1$, $\mathcal{U}_2$, and $\mathcal{U}_3$ receive energy at every $5$, $10$, and $20$ global rounds, respectively. 

{\bf Benchmarks.} 
% We compare Algorithm~\ref{Alg} with the following federated learning benchmarks.  
To evaluate the performance of Algorithm~\ref{Alg}, we consider the conventional federated learning algorithm from Section~\ref{federated} (known as \emph{FedAvg} \cite{mcmahan2017communication}), but under the constraint that users receive energy according to the energy arrival process in Section~\ref{sec:energy}, and implement two benchmarks with respect to the specific client scheduling policy. 
% Unlike the original \emph{FedAvg} setting, i scheduling is governed by the energy availability of the clients.   We then consider the two client scheduling policies. 

% Unlike the original \emph{FedAvg} setting, the scheduling is governed by the energy availability of the clients.   We then consider the two client scheduling policies. 


% We compare Algorithm~\ref{Alg} with the conventional federated learning setting from \cite{mcmahan2017communication}, also known as the federated averaging (\emph{FedAvg}) algorithm. 


\noindent
{\it Benchmark 1:} 
In the first benchmark, each client participates in training as soon as they have enough energy, and then waits until the next energy arrival. More specifically, as soon as $t\mod TE_i = 0$, the client participates in the current global round,  by updating the current state of the global model through $T$ local training iterations as in  \eqref{localupdate}, and then sending the local update to the server. The server then updates the global model according to  \eqref{eq:aggregation}. The client does not participate in training in the next $E_i-1$ global rounds, until the next energy arrival.  
% Note that in this setting clients do not scale the gradients with respect to the energy arrivals. 
% We first consider the federated setting algorithm from Section~\ref{sysmodel} when clients participate in training as soon as they have energy available, by computing a local update from \eqref{gradient} and sending it to the server, and then wait for the next energy arrival. Note that in this setting clients do not scale the gradients with respect to the energy arrivals. 


\noindent
{\it Benchmark 2:} 
In the second benchmark, the global model is updated only when all clients have received energy, i.e., the  server waits until all clients have energy available before initiating a global update. 
% and then the global is updated according to the standard \emph{FedAvg} algorithm. 
% In other words, the global model is updated only when all clients have energy available.  
% In other words, the global model is updated only when all clients have energy available. 
After all clients have received energy, the server sends the current state of the global model to the clients, the clients compute a local model as in \eqref{localupdate}, and then the server aggregates the local models to update the global model as in \eqref{eq:aggregation}. 
Note that in this case, the server needs to wait for the slowest client, hence the global model is updated once in the duration of $20$ global rounds. 

% updates the global model only when all clients have enough energy to participate in training. 
% In this case, the server waits until all clients have energy, then sends the current model parameters to the clients, clients compute the stochastic gradient from \eqref{gradient} and send it back to the server, and then the server updates the model as in \eqref{eq:aggregation}. 



% Finally, we also implement the conventional distributed SGD framework from Section~\ref{federated} when all clients are available at every iteration, which represents our target (desired) accuracy level.  
We evaluate the training performance in terms of the test accuracy with respect to the number of global rounds. 
Our results are given in Figure~\ref{fig:test-accuracy}. In our experiments, we also implement the original federated learning algorithm (\emph{FedAvg}) from Section~\ref{federated} without any resource limitations, which acts as an upper bound on the accuracy.  We observe that Algorithm~\ref{Alg} achieves an accuracy of $77\%$, which is comparable to the accuracy of {\it FedAvg}, whereas the accuracy of the two benchmarks are $60\%$ and $62\%$, respectively, within $1000$ global rounds. 
This is caused by the fact that, in the first benchmark, the training algorithm favors clients with more frequent energy availability, which causes the global model to be biased. In the second benchmark, the server waits until all clients have energy available before each global update, which causes the convergence to be very slow even though the algorithm is unbiased. On the other hand, Algorithm~\ref{Alg} converges fast and significantly outperforms the benchmarks in terms of test accuracy.  
% achieves the same accuracy level (about $80\%$) as conventional distributed SGD, whereas the two benchmarks achieve an accuracy of $64\%$ and $52\%$, respectively, within $t=1000$ iterations.


% We demonstrate our results in terms of the test accuracy with respect to time $t$ in Figure~\ref{fig:test-accuracy}. Our results show that Algorithm~\ref{Alg-deterministic} achieves the same accuracy level (about $80\%$) as conventional distributed SGD, whereas the two benchmarks achieve an accuracy of $64\%$ and $52\%$, respectively, within $t=1000$ iterations. This is due to the fact that the first benchmark favors clients with more frequent energy arrivals, hence the model is biased. The second benchmark waits for all clients to have enough energy before making a single SGD update, hence, even though the training algorithm is unbiased, its convergence rate is very slow. 
% In contrast, Algorithm~\ref{Alg-deterministic} converges fast while achieving good accuracy. 



